On the Equivalency, Substitutability, and Flexibility of Synthetic Data

We study, from an empirical standpoint, the efficacy of synthetic data in real-world scenarios. Leveraging synthetic data for training perception models has become a key strategy embraced by the community due to its efficiency, scalability, perfect annotations, and low costs. Despite proven advantages, few studies put their stress on how to efficiently generate synthetic datasets to solve real-world problems and to what extent synthetic data can reduce the effort for real-world data collection. To answer the questions, we systematically investigate several interesting properties of synthetic data -- the equivalency of synthetic data to real-world data, the substitutability of synthetic data for real data, and the flexibility of synthetic data generators to close up domain gaps. Leveraging the M3Act synthetic data generator, we conduct experiments on DanceTrack and MOT17. Our results suggest that synthetic data not only enhances model performance but also demonstrates substitutability for real data, with 60% to 80% replacement without performance loss. In addition, our study of the impact of synthetic data distributions on downstream performance reveals the importance of flexible data generators in narrowing domain gaps for improved model adaptability.

==> tables_algs/authoring_groups.tex <==
\begin{table*}[]
\setlength{\tabcolsep}{8.6pt}
% \small
\footnotesize
% \scriptsize
% \fontsize{9.5pt}{9.5pt}\selectfont
  \aboverulesep=0ex
  \belowrulesep=0ex 
%   \vspace{6pt}
\begin{center}
\setlength{\tabcolsep}{5.6pt}
\begin{tabular}{c|c|c|c|c}
\toprule
\textbf{Activity Name} & \textbf{Alignment} & \textbf{Face At} & \textbf{Atomic Actions} & \textbf{Other Conditions} \\
\midrule \midrule
\multirow{2}{*}{Walking} & \multirow{2}{*}{Straight Line, Circle, Rectangle} & \multirow{2}{*}{Same Direction} & \multirow{2}{*}{walk} &  \multirow{2}{*}{Adjust animation speed at runtime} \\
 & & & & \\
\hline
\multirow{2}{*}{Waiting} & \multirow{2}{*}{Multi-Row Straight Lines} & \multirow{2}{*}{Same Direction} & \multirow{2}{*}{idle, text, talk, point, wave} & \multirow{2}{*}{N/A} \\
 & & & & \\

\hline

\multirow{2}{*}{Queueing} & \multirow{1}{*}{Straight Line, One-Corner Line,} & \multirow{2}{*}{Front of Queue} & \multirow{2}{*}{idle, text, talk, point} & \multirow{2}{*}{N/A} \\
 & Two-Corner Line, Parabola, Curve & & & \\
\hline

\multirow{2}{*}{Talking} & \multirow{2}{*}{Circle} & \multirow{2}{*}{Group Center} & \multirow{2}{*}{talk} & \multirow{2}{*}{N/A} \\
 & & & & \\
\hline

\multirow{2}{*}{Dancing} & \multirow{2}{*}{Multi-Row Straight Lines} & \multirow{2}{*}{Same Direction} & \multirow{2}{*}{dance} & \multirow{2}{*}{Nearly-synchronous movements}  \\
& & & & \\

\hline

\multirow{2}{*}{Jogging} & \multirow{2}{*}{Straight Line, Circle, Rectangle} & \multirow{2}{*}{Same Direction} & \multirow{2}{*}{run} & \multirow{2}{*}{Adjust animation speed at runtime} \\
 & & & & \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-10pt}
\caption{Rules and adjustments for activity authoring.}
\label{tab:authoring_groups}
\end{table*}

==> tables_algs/col_avoid_alg.tex <==

\begin{algorithm}[t]
\caption{Dynamic speed adjustment for collision avoidance.}\label{alg:collision_avoidance}
\begin{algorithmic}[1]
\Require a list of instantiated characters and their initial animation speeds. 
\State At every frame,
\For{\textit{character} in Characters}
    \State \textit{init\_speed} $\gets$ Initial Speed of \textit{character}
    \State \textit{Speed} $\gets$ Current Speed of \textit{character}
    \State \textit{pos} $\gets$ Position of \textit{character} 
    \State \textit{forward} $\gets$ Forward Vector of \textit{character} 

    \State \textit{flag} $\gets$ False
    \For{\textit{other\_character} in Characters}
        \If{\textit{character} is not \textit{other\_character}}
            \State \textit{pos\_other} $\gets$ Position of \textit{other\_character} 
            \State \textit{offset} $\gets$ \textit{pos\_other} - \textit{pos}
            \State \textit{angle} $\gets$ Angle Between \textit{forward} and \textit{offset}
            \State \textit{dist} $\gets$ Length of \textit{offset}

            \If{\textit{dist} $\leq$ 0.8 $\And$ \textit{angle} $\leq$ 60}
                \State \textit{flag} $\gets$ True
            \EndIf
        \EndIf
    \EndFor
    \If{\textit{flag}}
            \State\textit{Speed} $\gets$ Max(\textit{Speed} * 0.96, 0.1) 
        \Else
            \State \textit{Speed} $\gets$ Min(\textit{Speed} * 1.03, \textit{init\_speed}) 

    \EndIf
\EndFor


\end{algorithmic}
\end{algorithm}


==> tables_algs/domain_randomization.tex <==

\begin{table*}[]
\setlength{\tabcolsep}{6.6pt}
% \small
\footnotesize
% \scriptsize
% \fontsize{9.5pt}{9.5pt}\selectfont
  \aboverulesep=0ex
  \belowrulesep=0ex 
%   \vspace{6pt}
\begin{center}
\setlength{\tabcolsep}{5.6pt}
\begin{tabular}{c|c|c|c}
\toprule
\textbf{Category} & \textbf{Randomizer} & \textbf{Variable} & \textbf{Distribution} \\
\midrule
\midrule
\multirow{2}{*}{Scenes} & Scene Selection  & scene & a set of prebuilt 3D environments \\
\cline{2-4}
 & HDRI Selection & hdri & a set of collected HDRIs
 \\

\midrule
\multirow{4}{*}{Camera} & \multirow{4}{*}{Camera Position } & radius & Uniform(6, 10) \\
 &  & camera rotation & Uniform(0, 360) \\
 &  & camera height & Uniform(1, 5) \\
 &  & perturbation & Cartesian[Uniform(-1, 1), 0 Uniform(-1, 1)] \\


\midrule
\multirow{6}{*}{Lights} & Lighting Volume & volume & a set of lighting volume conditions \\
\cline{2-4}
 & Light Type  & light type & a set of light types \\
\cline{2-4}
 & \multirow{2}{*}{Light Position } & XZ position & Cartesian[Uniform(-20, 20), 0, Uniform(-20, 20)] \\
 &  & height & Uniform(5, 10) \\
\cline{2-4}
 & Light Intensity  & intensity range & Uniform(0.5, 3) \\
\cline{2-4}
 & Light Rotation  & orientation range & Face at Cartesian[Uniform(-50, 50), 0 Uniform(-50, 50)] \\

\midrule
\multirow{4}{*}{Multi-Group} & Group Number  & group number range & UniformRange(1, MaxNumGroups) \\
\cline{2-4}
 & Group Selection  & group activity & a set of modular groups \\
\cline{2-4}
 & \multirow{2}{*}{Group Placement } & group position & Cartesian[Uniform(-20, 20), 0, Uniform(-20, 20)]
 \\
 &  & group rotation & Euler[0, Uniform(0, 360), 0] \\
 
\midrule
\multirow{14}{*}{\shortstack{Activity\\Authoring}} & Character Number  & character number range & UniformRange(1, MaxNumCharacters) \\
\cline{2-4}
 & Multi-person Subgroup  & multi-person number range & UniformRange(0, MaxNum) \\
\cline{2-4}
 & Character Selection  & character & a set of 2200 characters \\
\cline{2-4}
 & \multirow{2}{*}{Character Texture } & body color & RGBA[Uniform(0.4, 1), Uniform(0.4, 1), Uniform(0.4, 1), Uniform(0.6, 1)] \\
 &  & clothes colors & HSV[Uniform(0, 1), Uniform(0, 1), Uniform(0.4, 1)] \\
\cline{2-4}
 & Character Alignment  & alignment method & a set of aligment methods \\
\cline{2-4}
 & Character Interval  & interval & Uniform(MinInterval, MaxInterval) \\
\cline{2-4}
 & \multirow{2}{*}{Character Perturbation } & position perturbation & Uniform(-0.25*interval, 0.25*interval)  \\
 &  & rotation perturbation & Uniform(-45$^{\circ}$, 45$^{\circ}$) \\
\cline{2-4}
 & Atomic Action  & atomic action & a set of permitted atomic actions \\
\cline{2-4}
 & \multirow{4}{*}{Animation } & animation clip & a set of animation clips \\
 &  & blended parameter & Uniform(0, 1) \\
 &  & speed & Uniform(0.8, 1.2) \\
 &  & normalized starting time & Uniform(0, 1) \\


\bottomrule
\end{tabular}
\end{center}
\vspace{-10pt}
\caption{List of randomizers, variables, and distributions used in  {\datagenerator}.}
 \vspace{-10pt}
\label{tab:domain_randomization}
\end{table*}


